Datacenter Ethernet and RDMA: Issues at Hyperscale

We observe that emerging artificial intelligence, high-performance computing, and storage workloads pose new challenges for large-scale datacenter networking. RDMA over Converged Ethernet (RoCE) was an attempt to adopt modern Remote Direct Memory Access (RDMA) features into existing Ethernet installations. Now, a decade later, we revisit RoCE's design points and conclude that several of its shortcomings must be addressed to fulfill the demands of hyperscale datacenters. We predict that both the datacenter and high-performance computing markets will converge and adopt modernized Ethernet-based high-performance networking solutions that will replace TCP and RoCE within a decade.

==> Makefile <==
DOCUMENT=$(shell ls -1 *tex | sed -e "s/\.tex//")

FILES=*.tex 

all: $(DOCUMENT).pdf

$(DOCUMENT).pdf: $(FILES)
	if [ -f plt/Makefile ]; then make -C plt; fi
	if [ -f img/Makefile ]; then make -C img; fi
	if [ -d ../img ]; then make -C ../img; fi
	rm -f pdflatex.out
#	cd ppt && sh ./crop_all.sh
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	if grep -q citation $(DOCUMENT).aux; then bibtex $(DOCUMENT); fi;
# don't use pdflatex due to transparency issues  
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
# use ps2pdf to avoid lossy image compression in pdf which looks ugly on the
# beamer
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps

copyin: ~/projekte/latex/macros/*
	cp ~/projekte/latex/macros/bibliography.bib .
	cp ~/projekte/latex/macros/htor.sty .
	cp ~/projekte/latex/macros/htor_paper.cls .

show: $(DOCUMENT).pdf
	atril $(DOCUMENT).pdf

spell:
	ln -sf ~/projekte/templates/aspell.en_US.dic .
	for i in $$(ls -1 *.tex); do \
		echo "checking $$i ... "; \
		aspell -t --lang=en_US --home-dir="$$(pwd)" -p aspell.en_US.dic -c $$i; \
done; \

force:
	touch $(DOCUMENT).tex
	make $(DOCUMENT).pdf

clean:
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	rm -f *.aux *.out sparsity.synctex.gz
	rm -f $(DOCUMENT).blg $(DOCUMENT).dvi $(DOCUMENT).vrb comment.cut
	rm -f $(DOCUMENT).pdf $(DOCUMENT).toc $(DOCUMENT).lo[a,f,g,h,l,t]
	rm -f $(DOCUMENT).nav $(DOCUMENT).snm $(DOCUMENT).ps $(DOCUMENT).out
	rm -f aspell*dic
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	if [ -d img ]; then make -C img clean; fi
	if [ -d slides ]; then make -C img clean; fi
	if [ -d ../img ]; then make -C ../img clean; fi

pack: $(DOCUMENT).tgz

$(DOCUMENT).tgz: *.tex
	if [ -d $(DOCUMENT) ]; then rm -r $(DOCUMENT); fi
	mkdir $(DOCUMENT) 
	cp *.tex $(DOCUMENT)
	cp *.sty $(DOCUMENT)
	cp *.cls $(DOCUMENT)
	cp *.bib $(DOCUMENT)
	cp *.pdf $(DOCUMENT)
	if [ -d img ]; then cp -a img $(DOCUMENT); fi
	if [ -d kivio ]; then cp -a kivio $(DOCUMENT); fi
	cp Makefile $(DOCUMENT)
	make -C $(DOCUMENT)
	cp $(DOCUMENT)/$(DOCUMENT).pdf $(DOCUMENT)/$(DOCUMENT)_orig.pdf
	make -C $(DOCUMENT) clean
	tar czf $(DOCUMENT).tgz $(DOCUMENT) 
	tar tzf $(DOCUMENT).tgz
	rm -fr $(DOCUMENT)
	@echo "voila: $(DOCUMENT).tgz"

commit: clean 
	svn commit

count: $(DOCUMENT).pdf
	pdftotext $(DOCUMENT).pdf -|wc -w

update: clean 
	svn update


